Skeleton-DML: Deep Metric Learning for Skeleton-Based One-Shot Action Recognition

One-shot action recognition allows the recognition of human-performed actions with only a single training example. This can influence human-robot-interaction positively by enabling the robot to react to previously unseen behaviour. We formulate the one-shot action recognition problem as a deep metric learning problem and propose a novel image-based skeleton representation that performs well in a metric learning setting. Therefore, we train a model that projects the image representations into an embedding space. In embedding space the similar actions have a low euclidean distance while dissimilar actions have a higher distance. The one-shot action recognition problem becomes a nearest-neighbor search in a set of activity reference samples. We evaluate the performance of our proposed representation against a variety of other skeleton-based image representations. In addition, we present an ablation study that shows the influence of different embedding vector sizes, losses and augmentation. Our approach lifts the state-of-the-art by 3.3% for the one-shot action recognition protocol on the NTU RGB+D 120 dataset under a comparable training setup. With additional augmentation our result improved over 7.7%.

==> common_packages.tex <==

\usepackage{iccv}
% \usepackage{times}
% \usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{subfig}
% \usepackage{tabularx}
% \usepackage{multirow}

\usepackage{booktabs}
\usepackage{graphicx}

% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}
\usepackage{xparse}
% \usepackage{notation}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{color}
\usepackage{pgfplots} 
\setlength {\marginparwidth }{2cm} 
\usepackage{todonotes}
% \usepackage<r{flushend}

\setlength{\textfloatsep}{1.2em}
\setlength{\dbltextfloatsep}{1.2em}
\usepackage[font=small]{caption}


\usepackage{notation_memmesheimer}
\usepackage{hyperref}
\usepackage{lipsum}
\input{00_defines}
\usepackage[detect-none]{siunitx}
\sisetup{range-phrase = \text{--}}

\pgfplotsset{width=.7\linewidth,compat=1.9}


\graphicspath{{images/}}

\usepackage[acronym]{glossaries}
\newacronym{har}{HAR}{Human Action Recognition}
\newacronym{gnn}{GNN}{Graph Neural Network}
\newacronym{gcn}{GCN}{Graph Convolutional Network}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{rnn}{RNN}{Recurrent Neural Network}
\newacronym{gft}{GFT}{Graph Fourier Transform}
\newacronym{imu}{IMU}{Inertial Measurement Unit}
\newacronym{mlp}{MLP}{Multilayer Perceptron}
\newacronym{lstm}{LSTM}{Long Short-Term Memory}
\newacronym{gru}{GRU}{Gated Recurrent Unit}
\newacronym{sgd}{SGD}{Stochastic Gradient Descent}
\newacronym{adam}{ADAM}{Adaptive Moment Estimation}
\newacronym{ca}{CA}{Cosine Annealing}
\newacronym{cawr}{CAWR}{Cosine Annealing with Warm Restarts}
\makeglossaries

\newcommand{\figname}{Figure\ }
\newcommand{\tabname}{Table\ }
\newcommand{\utdmhad}{UTD-MHAD}
\newcommand{\mmact}{MMACT}
\newcommand{\approachname}{MMARGCN}
\newcommand{\githuburl}{\url{https://github.com/mduhme/mmargcn}}
\newcommand{\todo}[2][]{\textcolor{red}{#2}}
